Safety Index Synthesis via Sum-of-Squares Programming

Control systems often need to satisfy strict safety requirements. Safety index provides a handy way to evaluate the safety level of the system and derive the resulting safe control policies. However, designing safety index functions under control limits is difficult and requires a great amount of expert knowledge. This paper proposes a framework for synthesizing the safety index for general control systems using sum-of-squares programming. Our approach is to show that ensuring the non-emptiness of safe control on the safe set boundary is equivalent to a local manifold positiveness problem. We then prove that this problem is equivalent to sum-of-squares programming via the Positivstellensatz of algebraic geometry. We validate the proposed method on robot arms with different degrees of freedom and ground vehicles. The results show that the synthesized safety index guarantees safety and our method is effective even in high-dimensional robot systems.

==> orig_intro.tex <==
\section{Introduction}
Energy-function-based algorithms~\cite{zhao2021issa} have been widely studied as appealing tools for safe control. When properly designed, the energy function (also called the safety index or barrier function) maps danger states to high values and safe states to low values. Then safety can be ensured by finding a control that dissipates the energy. However, when control limits exist, the desired safe control may not be realizable, which breaks down the safety guarantee. Therefore, it is important to account for control limits.

Designing safety index is challenging. Because we have to ensure the existence of safe control for infinitely many states. The presence of control limits makes the problem even harder where the complex constraints depend on system dynamics, control limits, and safety requirements. Many existing works leverage special structures of systems to guarantee safety, such as kinematic bicycle~\cite{zhao2021issa}, Euler-Lagrange system~\cite{cortez2020safe}, and polynomial systems~\cite{zhao2021issa}. Another approach is to formulate 
% this 
safety index synthesis
as an optimization problem of a parameterized safety index. However, these methods do not scale well to high dimensional systems~\cite{clark2021control,wei2022safe}.

Sum-of-Squares Programming (SOSP) is a powerful tool and has been applied to safety index synthesis~\cite{clark2021verification, clark2021control, ames2019control} since it is a widely adopted approach to formally deal with optimization problems with infinitely many constraints. Existing SOSP-based safety index synthesis approaches try to design safety index such that there exists safe control for all states in the set of real numbers~\cite{ames2019control}. This type of constraint is known as \textit{global positiveness} constraint~\cite{zhao2022provably}. 
% However, \cite{clark2021control} points out that existing SOSP-based methods are inapplicable for synthesizing safety index. \cite{clark2021verification} requires polynomial control systems and does not scale to high-dimensional systems. \cite{ames2019control} requires a nominal controller, and the formulated problem is inefficient to solve.

In this work, we highlight that instead of satisfying \textit{global positiveness} constraints, safety index synthesis simply needs to satisfy \textit{local manifold positiveness} constraints, which enables the corresponding safety index design much less conservative. Subsequently, we propose a general, scalable, efficient SOSP-based method to transform
% to solve the \textit{local manifold positiveness} constraints, which transforms 
safety index synthesis problem into a nonlinear programming problem that can be solved efficiently by off-the-shelf solvers. 
% for safety index synthesis. Our proposed method will transform the safety index synthesis problem into a \textit{Local Manifold Positiveness Problem}. Then, we leverage the theory behind SOSP to construct the corresponding \textit{Refute Problem}, which is further
% simplified to a nonlinear programming problem that can be solved efficiently by off-the-shelf solvers. 
The experiments show that the synthesized safety index ensures the existence of safe control, and our method is time-efficient, robust, and optimal even in high-dimensional robot systems.

\textbf{Our contributions} We propose a novel SOSP-based method that can efficiently synthesize the safety index. The state-of-the-art SOSP-based methods are (i) limited to polynomial control systems~\cite{ames2019control}; (ii) hard to scale to high-dimensional systems (e.g., iteratively solving $\mathcal{O}(2k)$ SOS programs at $k$-th iteration~\cite{clark2021control}); (iii) limited to conservative solutions due to considering \textit{global positiveness} constraints. Our algorithm (i) is applicable to general nonlinear control systems; (ii) scales well to high-dimensional systems (solving only one nonlinear programming problem) and (iii) gives nonconservative solutions via solving \textit{local manifold positiveness} constraints. 
We show how the theoretical results transfer to a practical algorithm with safety guarantees and apply it to safety index synthesis for complex robot systems.
